PILLOW: Enhancing Efficient Instruction Fine-tuning via Prompt Matching

Instruction fine-tuning has conventionally been employed to adapt Large Language Models (LLMs) to a variety of tasks. Nonetheless, this technique often necessitates substantial computational resources, making it impractical for deployment by individuals or small-scale entities. Recently, Low-Rank Adaptation (LoRA) has become a promising alternative, offering high capabilities on par with full tuning with reduced resource overhead. However, attaining satisfactory performance through the fine-tuning of LoRA is a non-trivial challenge. In this paper, we propose PILLOW, which aims to improve LoRA's performance by a discrimination-based prompting method, leveraging LLMs' In-Context Learning ability. PILLOW incorporates a matching network that selects prompts from a user-defined prompt pool, concatenates the selected prompts with the user instruction as input, and performs inference using the LoRA-fine-tuned LLMs. Trained with Reinforcement Learning, PILLOW exhibits commensurate performance on various evaluation metrics compared with typical instruction fine-tuning methods, utilizing only consumer-grade GPU resources and exhibiting a large reduction in computational costs.

==> additions/acknowledgements.tex <==
\section*{Acknowledgements}
This document has been adapted by Yue Zhang, Ryan Cotterell and Lea Frermann from the style files used for earlier ACL and NAACL proceedings, including those for 
ACL 2020 by Steven Bethard, Ryan Cotterell and Rui Yan,
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> tabs/alpaca.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{llllll}
\toprule[2pt]
\textbf{Model}               & \textbf{Method}      & \textbf{ChatGPT Score} & \textbf{Perplexity} & \textbf{Reward} & \textbf{Manual Score} \\ \midrule[1pt]
\multirow{4}{*}{Bloomz-560m} & -                    & 2.71                   & 192.24              & 4.87            &                       \\
                             & SFT                  & 2.87                   & 106.07              & 5.30            &                       \\
                             & LoRA                 & 2.56                   & 149.93              & 4.89            &                       \\ \cline{2-6} 
                             & \ours & 2.63 \textcolor{red}{(+0.07)}    & 140.57 \textcolor{red}{(-9.36) }     & 4.68 \textcolor{blue}{(-0.21)}   &                       \\ \hline
\multirow{4}{*}{Bloomz-1b1}  & -                    & 3.01                   & 108.2               & 5.71            &                       \\
                             & SFT                  & 3.29                   & 52.02               & 6.48            &                       \\
                             & LoRA                 & 3.09                   & 78.81               & 5.83            &                       \\ \cline{2-6} 
                             & \ours & 3.21 \textcolor{red}{(+0.12)}          & 67.36 \textcolor{red}{(-11.45)}      & 5.89 \textcolor{red}{(+0.06)}    &                       \\ \hline
\multirow{4}{*}{Bloomz-7b1}  & -                    & 3.14                   & 161.19              & 5.88            &                       \\
                             & SFT                  & 3.84                   & 64.34               & 6.49            &                       \\
                             & LoRA                 & 3.27                   & 120.70              & 5.94            &                       \\ \cline{2-6} 
                             & \ours & 3.76 \textcolor{red}{(+0.49)}           & 103.65 \textcolor{red}{(-17.05)}     & 6.07 \textcolor{red}{(+0.13)}    &                       \\ \bottomrule[2pt]
\end{tabular}
\caption{Results on Alpaca.}
\label{tab:alpaca}
\end{table*}

==> tabs/dolly.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{llllll}
\toprule[2pt]
\textbf{Model}               & \textbf{Method} & \textbf{ChatGPT Score} & \textbf{Perplexity} & \textbf{Reward} & \textbf{Manual Score} \\ \midrule[1pt]
\multirow{4}{*}{Bloomz-560m} & -               & 2.83                   & 247.45              & 4.26            &                       \\
                             & SFT             & 3.01                   & 218.61              & 5.01            &                       \\
                             & LoRA            & 2.64                   & 221.16              & 4.34            &                       \\ \cline{2-6} 
                             & \ours            & 2.74 \textcolor{red}{(+0.1)}            & 191.9 \textcolor{red}{(-29.26)}      & 4.70 \textcolor{red}{(+0.36)}    &                       \\ \hline
\multirow{4}{*}{Bloomz-1b1}  & -               & 3.13                   & 227.43              & 4.74            &                       \\
                             & SFT             & 3.37                   & 67.93               & 5.87            &                       \\
                             & LoRA            & 3.08                   & 140.40              & 4.79            &                       \\ \cline{2-6} 
                             & \ours            & 3.31 \textcolor{red}{(+0.23)}           & 112.78 \textcolor{red}{(-27.62)}     & 5.31 \textcolor{red}{(+0.52)}    &                       \\ \hline
\multirow{4}{*}{Bloomz-7b1}  & -               & 3.24                   & 244.09              & 4.86            &                       \\
                             & SFT             & 3.89                   & 56.64               & 5.61            &                       \\
                             & LoRA            & 3.33                   & 146.92              & 4.93            &                       \\ \cline{2-6} 
                             & \ours            & 3.81 \textcolor{red}{(+0.48)}           & 113.09 \textcolor{red}{(-33.83)}     & 5.08 \textcolor{red}{(+0.15)}    &                       \\ \bottomrule[2pt]
\end{tabular}
\caption{Results on Dolly.}
\label{tab:dolly}
\end{table*}
